An extended framework for characterizing social robots

Social robots are becoming increasingly diverse in their design, behavior, and usage. In this chapter, we provide a broad-ranging overview of the main characteristics that arise when one considers social robots and their interactions with humans. We specifically contribute a framework for characterizing social robots along 7 dimensions that we found to be most relevant to their design. These dimensions are: appearance, social capabilities, purpose and application area, relational role, autonomy and intelligence, proximity, and temporal profile. Within each dimension, we account for the variety of social robots through a combination of classifications and/or explanations. Our framework builds on and goes beyond existing frameworks, such as classifications and taxonomies found in the literature. More specifically, it contributes to the unification, clarification, and extension of key concepts, drawing from a rich body of relevant literature. This chapter is meant to serve as a resource for researchers, designers, and developers within and outside the field of social robotics. It is intended to provide them with tools to better understand and position existing social robots, as well as to inform their future design.

==> sec_role.tex <==
One of the relevant dimensions that shapes human-robot interaction is the \textit{role} that the robot is designed to fulfill.
The concept of role is an abstract one, for which various different perspectives can be presented. 
In this section, we specifically look at the \textit{relational role} of the robot towards the human.
This is the role that a robot is designed to fulfill within an interaction, and is not specifically tied to an application area.
 
Towards clarifying the concept of relational role, it is important to immediately distinguish relational role from role in an activity or application. 
In a specific activity or application, we may expect to find activity-specific roles (as in role-playing), such as teacher, driver, game companion, cook, or therapist. 
These types of roles are defined by the type of activity performed between the robot and humans, therefore making it an open-ended list that is likely to stay in constant evolution, as robots become applied to new fields and tasks.

%Given this prime distinction, it is also important to rule out other concepts that what we do not mean by the term \textit{relational role}. 
%remove bullets and bolds from anything that is not what WE want to emphasize
%say that we will look into previous examples from literature, explain why they are fuzzy and HCI-directed, and that we will aglomerate them into a more general taxonomy that can superclass/superseed the existing ones
%motivar que 
%merge this into the previous paragraph

%Before moving on with the discussion about relational roles, we highlight and define the following terms in order to clarify their distinction from the concept of relational role:
%\begin{description}
%\item[\textbf{Activity/Application domain}] is the actual task or activity in which both robots and humans participant and interact. 
%Examples of activities would be: assembling a piece of furniture, cooking a meal, learning a second language, playing a game, painting a picture, etc.
%\item[\textbf{Application role}] is the activity and task-directed part that the robot takes within the application domain. 
%It is related with role-playing, and specifically defined within a task. Examples of application roles are: Teacher, Driver, Game-Player, Cook, Mechanic, Therapist, Receptionist, etc.
%\item[\textbf{Application area/field}] is a broader definition of the application domain. 
%Various different application roles are likely to be contained within an application field. 
%#These application fields allow to cluster various types of application into general groups such as Urban Search and Rescue (USAR), Social assistance, Education, Home assistance, Entertainment, assistance in Space, etc.
%\item[\textbf{Product-lifetime role}] refers to the role of humans within the various stages of the lifetime of a robot as a product. 
%Examples of these roles would be Programmers, Designers, Interaction-Designers, Manufacturer, Operator, End-User, etc. 
%\end{description}

Given the fuzziness of this concept, there have not been many attempts at generalizing the concept of role of robots within a relation with humans. 
For the rest of this section, we will present and analyze some broader definitions from the existing literature, to conclude by contributing a broad classification that attempts to agglomerate the main concepts of the pre-existing ones in a way that it can contain and supersede them.

Scholtz et al. presented a list of interaction models found in \ac{HRI} \cite{Scholtz2003}. They included roles that humans may have towards a robot in any \ac{HRI} application. The list defines the roles of the Supervisor, who monitors and controls the overall system (single or multiple robots), while acting upon the system's goals/intentions; the Operator, who controls the task indirectly, by triggering actions (from a set of pre-approved ones), while determining if these actions are being carried out correctly by the robot(s); the Mechanic, who is called upon to control the task, robot and environment directly, by performing changes to the actual hardware of physical set-up; the Peer, who takes part in the task or interaction, while suggesting goals/intentions for the supervisor to perform; 
and the Bystander, who may take part in the task or interaction through a subset of the available actions, while most likely to not have been previously informed about which those are.

These five roles were initially adapted from \ac{HCI} research, namely from Norman's \ac{HCI} Model \cite{Norman1986}. 
As such, they refer mostly to the role of the human within a technological system, whereas in this section we look for a classification to support the roles of robots in relation with humans within their interaction with each other.

Later, Goodrich \& Schultz built upon this list to propose a classification of roles that robots can assume in \ac{HRI} \cite{goodrich2008human}. In Goodrich \& Schultz’s list, it is not specified whether the role refers to a human or to a robot. 
Their proposed classification can be misleading, as they take Scholtz’s roles (for humans) and directly apply them to both robots and humans with no discussion provided. They also extended the list by adding two more roles, but these are defined only for robot. In the Mentor role, the robot is in a teaching or leadership role for the human; in the Informer role, the robot is not controlled by the human, but the human uses information coming from the robot in, for example, a reconnaissance task.

The concept of robot roles was also addressed by Breazeal \cite{Breazeal2004}, who proposed four interaction paradigms of \ac{HRI}. In this paradigms, the robot can either take a role of a Tool, directed at performing specific tasks, with various levels of autonomy; a Cyborg extension, in which it is physically merged with the human in a way that the person accepts it as an integral part of their body; an Avatar, through which the person can project him/herself in order to communicate with another from far away; or a Sociable partner, as in classic science-fiction fantasy.

Based on the many different proposed classifications, and of all the various interaction scenarios and applications found throughout literature, and presented throughout this chapter, we have outlined our own classification for the role of robots within a relation with humans. Our classification attempts to merge the various dimensions of interaction while steeping away from explicit types of scenarios or applications. It does not necessarily add or propose new roles, but instead, redefines them from a relational perspective, placing emphasis on how the robot relates from a human's perspective, as depicted in Figure~\ref{fig:roles}.

\begin{figure*}
    \centering
    \includegraphics[width=0.95\textwidth]{Figures/robot_roles.png}
    \caption{Our classification of relational roles of robots towards humans.}
    \label{fig:roles}
\end{figure*}

%for you
%service robot, autonomous cars

%as you
%avatars, tele-presence

%with you
%tele-operated assistive robot, symbiotic co-bot.

%as if you
%research tools

%around you
%co-operative, co-present, or bystanders

%as part of you
%strength-enhancing exoskeletons, robotic limbs
% repreference on wearbales (maybe contains nice references in the paper as well): http://shape.stanford.edu/research/rovables/Rovables_UIST_2016.pdf

%merge these bullets with the paragraphs
In our classification for relational roles of robots, we view \ac{HRI} as including both \textbf{robot} and \textbf{you}. 
As such, we consider the following roles that a \textit{robot} may have towards \textit{you}:
\begin{itemize}
\item A robot \textbf{for you} serves some utility on a given task.
This is the most traditional role of a tool or a servant, that a robot may have towards a human, and is inspired by most previous classifications. 
Despite closely related with the concept of a tool, as proposed by other authors, we frame this role as a more broader type of robotic tool, which can even include, e.g., autonomous cars.
\item A robot \textbf{as you} represents you somehow, namely, but not limited to, tele-presence. However it does not necessarily imply interaction from far away as in Breazeal's classification \cite{Breazeal2004}.
This type of role can exist even when inter-actors are co-located, as long as the robot is acting in place of another person who operates it (e.g. shared autonomy).
\item A robot \textbf{with you} typically collaborates with you, with various levels of autonomy, including being part of a group with you. 
It is used in applications in which both humans and robots act together, as a team, or towards common goals. 
The robot and human are not necessarily co-located, and can include, e.g. e tele-operated assistive robot or a symbiotic co-bot.
\item A robot \textbf{as if you} gave it particular social or psychological traits, in order to be used as a research tool. 
This is a particular role which has also been mentioned in Fong's survey \cite{fong2003survey}. 
Robots are increasingly being used as research tools to perform a wide range of comparative studies. 
To date, robots have been used to examine, validate and refine theories of social and biological development, psychology, neurobiology, emotional and non-verbal communication, and social interaction.
\item A robot \textbf{around you}, sharing the same physical space and common resources.
It differs from a \textit{robot with you} by referring to robots that are necessarily co-located with humans, but to not necessarily collaborate with them. 
These are typically called e.g., co-operating, co-present, or bystanders as previously proposed in Scholzt's classification \cite{Scholtz2003}.
\item A robot \textbf{as part of you} extends your human body's capabilities. 
These robots typically have nonexistent or very limited autonomy, but provide humans with physical capabilities that they could otherwise not perform using their own biological body. Such robots can be used for pure embodiment extension (e.g. strength-enhancing exoskeletons), or to fill in motive and perceptive defects and injuries (e.g. using robotic limbs after amputation, or an artificial hearing aid).
\end{itemize}

The list of relational roles that we present defines non-exclusive roles, meaning that for some particular applications, we may design and develop robots that take more than one of these roles, or take a different role when more than one human is involved in the interaction.
An example would be of a robot used in an office, which can be used \textit{for the users} to deliver mail and packages to different locations, while at the same time, is a robot that behaves \textit{around the users}, while navigating the office space. Another example would be an autonomous vehicle operating \textit{for} the passenger(s), but \textit{around} the pedestrians and human drivers.


%To clarify their taxonomy, they present a table containing examples of roles between robots and humans that can arise in several application area. This table is cited verbatim in Table~\ref{tab:hriRoles}.
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
%\begin{table}[]
%\caption{Taxonomy for HRI roles proposed by Goodrich \& Schultz \cite{goodrich2008human}}
%\label{tab:hriRoles}
%\resizebox{\textwidth}{!}{%
%\begin{tabular}{lll}
%\hline\noalign{\smallskip}
%Application area                     & Role                            & Example                                    \\ 
%\noalign{\smallskip}\svhline\noalign{\smallskip}
%\multirow{2}{*}{Search and Rescue}   & Human is supervisor or operator & Remotely operated search robots            \\
%                                     & Human and robot are peers       & Robot supports unstable structures         \\ \midrule
%Assistive Robotics                   & Human and robot are peers,      & Assistance for the blind,                  \\
%                                     & \hspace{1cm}or robot is tool                & \hspace{1cm}and therapy for the elderly                \\
%                                     & Robot is mentor                 & Social interaction for autistic children   \\ \midrule
%\multirow{3}{*}{Military and Police} & Human is supervisor             & Reconnaissance, de-mining                  \\
%                                     & Human and robot are peers       & Patrol Support                             \\
%                                     & Human is information consumer   & Commander using reconnaissance information \\ \midrule
%\multirow{3}{*}{Edutainment}         & Robot is mentor                 & Robotic classroom assistant                \\
%                                     & Robot is mentor                 & Robotic museum tour guide                  \\
%                                     & Robot is peer                   & Social companion                           \\ \midrule
%\multirow{2}{*}{Space}               & Human is supervisor or operator & Remote science and exploration             \\
%                                     & Human and robot are peers       & Robotic astronaut assistant                \\ \midrule
%\multirow{3}{*}{Home and industry}   & Human and robot are peers       & Robotic companion                          \\
%                                     & Human is supervisor             & Robotic vacuum                             \\
%                                     & Human is supervisor             & Robot construction                         \\
%\noalign{\smallskip}\hline\noalign{\smallskip}
%\end{tabular}%
%}
%\end{table}

